Treating Detector Systematics via a Likelihood Free Inference Method

Estimating the impact of systematic uncertainties in particle physics experiments is challenging, especially since the detector response is unknown analytically in most situations and needs to be estimated through Monte Carlo (MC) simulations. Typically, detector property varia-tions are parameterized in ways that implicitly assume a specific physics model, which can introduce biases on quantities measured by an analysis. In this paper, we present a method to recover a model-independent, event-wise estimation of the detector response variation by applying a likelihood-free inference method to a set of MC simulations representing discrete detector realizations. The method provides a re-weighting scheme for every event, which can be used to apply the effects of detector property variations fully decoupled from the assumed physics model. Using a toy MC example inspired by fixed-baseline neutrino oscillation experiments, we demonstrate the performance of our method. We show that it fully decouples the modeling of the detector response from the physics parameters to be measured in a MC forward-folding analysis.

==> figures/detector_response.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{cornflowerblue86180233}{RGB}{86,180,233}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{gray}{RGB}{128,128,128}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{orange2301590}{RGB}{230,159,0}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={reconstructed energy (GeV)},
xmajorgrids,
xmin=-2.5, xmax=52.5,
xtick style={color=black},
y grid style={darkgray176},
ylabel={density},
ymajorgrids,
ymin=-0.00508741986493034, ymax=0.106835817163537,
ytick style={color=black}
]
\addplot [very thick, black]
table {%
0 0
0.505050505050505 1.33644351922508e-73
1.01010101010101 7.99175740533176e-49
1.51515151515152 9.50336816689251e-37
2.02020202020202 2.90323142443127e-29
2.52525252525253 4.46581178684688e-24
3.03030303030303 3.06681744445662e-20
3.53535353535354 2.81237896768507e-17
4.04040404040404 6.40720619983322e-15
4.54545454545455 5.3152373074917e-13
5.05050505050505 2.06236202569939e-11
5.55555555555556 4.44445799412e-10
6.06060606060606 6.01237383875749e-09
6.56565656565657 5.58579122120867e-08
7.07070707070707 3.81357622071682e-07
7.57575757575758 2.01558657209221e-06
8.08080808080808 8.59020299628187e-06
8.58585858585859 3.04951595596502e-05
9.09090909090909 9.25660468841755e-05
9.5959595959596 0.000245441062652847
10.1010101010101 0.000578598191996657
10.6060606060606 0.00123061864089687
11.1111111111111 0.00239083937353028
11.6161616161616 0.00428747115960641
12.1212121212121 0.00716063783619338
12.6262626262626 0.0112235334725765
13.1313131313131 0.0166191586261132
13.6363636363636 0.0233822297345745
14.1414141414141 0.0314151184429379
14.6464646464646 0.0404834521466917
15.1515151515152 0.0502324813686224
15.6565656565657 0.0602209178269367
16.1616161616162 0.0699658047538338
16.6666666666667 0.078990655886556
17.1717171717172 0.0868695508338961
17.6767676767677 0.0932616327900722
18.1818181818182 0.0979328642054947
18.6868686868687 0.100764331834664
19.1919191919192 0.101748397298607
19.6969696969697 0.100975323021872
20.2020202020202 0.0986136246571512
20.7070707070707 0.094887409955472
21.2121212121212 0.0900535352050883
21.7171717171717 0.0843807354003578
22.2222222222222 0.0781321317862137
22.7272727272727 0.0715518153359965
23.2323232323232 0.0648556235050562
23.7373737373737 0.0582258035567788
24.2424242424242 0.0518089895943357
24.7474747474747 0.0457167920410102
25.2525252525253 0.0400282772191495
25.7575757575758 0.0347936679949867
26.2626262626263 0.0300386940871522
26.7676767676768 0.0257691380520096
27.2727272727273 0.02197524213052
27.7777777777778 0.0186357502516249
28.2828282828283 0.0157214519623303
28.7878787878788 0.0131981683299144
29.2929292929293 0.0110291741517868
29.7979797979798 0.00917708803941736
30.3030303030303 0.00760528491032163
30.8080808080808 0.00627889718677657
31.3131313131313 0.00516547449142814
31.8181818181818 0.00423536942096403
32.3232323232323 0.00346191118425829
32.8282828282828 0.002821421151305
33.3333333333333 0.00229311587582342
33.8383838383838 0.00185893475400387
34.3434343434343 0.00150332168785387
34.8484848484849 0.00121298322571565
35.3535353535354 0.000976639778523546
35.8585858585859 0.000784781667282243
36.3636363636364 0.000629437881483163
36.8686868686869 0.000503962415213427
37.3737373737374 0.000402840774810309
37.8787878787879 0.000321517593476177
38.3838383838384 0.000256245125523392
38.8888888888889 0.000203951619374759
39.3939393939394 0.000162128092373201
39.8989898989899 0.000128731775365999
40.4040404040404 0.000102104398912977
40.9090909090909 8.09035068268079e-05
41.4141414141414 6.4045068822016e-05
41.9191919191919 5.06557939488219e-05
42.4242424242424 4.00336994712183e-05
42.9292929292929 3.16156512211205e-05
43.4343434343434 2.49507512178329e-05
43.9393939393939 1.96786000313897e-05
44.4444444444444 1.55116011604893e-05
44.949494949495 1.22206006488114e-05
45.4545454545455 9.62326664965862e-06
45.959595959596 7.57471091860464e-06
46.4646464646465 5.95993807150605e-06
46.969696969697 4.68778001332801e-06
47.4747474747475 3.68603349571401e-06
47.979797979798 2.89756960957749e-06
48.4848484848485 2.27722643767425e-06
48.989898989899 1.78933127290096e-06
49.4949494949495 1.40572783494802e-06
50 1.10420775638829e-06
};
\addlegendentry{$\mu = 1$, $\sigma=0.2$}
\addplot [very thick, orange2301590]
table {%
0 0
0.505050505050505 5.8459672582287e-33
1.01010101010101 4.08771362227103e-22
1.51515151515152 7.5931715656652e-17
2.02020202020202 1.37303400455532e-13
2.52525252525253 2.45010145343584e-11
3.03030303030303 1.12313866850867e-09
3.53535353535354 2.13725667337357e-08
4.04040404040404 2.2154342781725e-07
4.54545454545455 1.47864794626697e-06
5.05050505050505 7.08918100122164e-06
5.55555555555556 2.63176015627645e-05
6.06060606060606 7.9803197736681e-05
6.56565656565657 0.000205564182320334
7.07070707070707 0.000463280302069635
7.57575757575758 0.000934461926359328
8.08080808080808 0.00171716961877122
8.58585858585859 0.00291562426531135
9.09090909090909 0.00462659021363582
9.5959595959596 0.00692526196401264
10.1010101010101 0.00985337040624205
10.6060606060606 0.013411521509577
11.1111111111111 0.0175567322073497
11.6161616161616 0.0222050774873504
12.1212121212121 0.0272385481449776
12.6262626262626 0.0325147465012829
13.1313131313131 0.0378779128379698
13.6363636363636 0.0431699050679934
14.1414141414141 0.0482400484728059
14.6464646464646 0.0529531356144231
15.1515151515152 0.057195214304993
15.6565656565657 0.0608771059275087
16.1616161616162 0.0639358242265882
16.6666666666667 0.0663342116808841
17.1717171717172 0.0680591848555186
17.6767676767677 0.0691189963108312
18.1818181818182 0.0695398952979469
18.6868686868687 0.0693625182362517
19.1919191919192 0.0686382759198578
19.6969696969697 0.0674259374509515
20.2020202020202 0.0657885478395235
20.7070707070707 0.0637907611279416
21.2121212121212 0.0614966257466395
21.7171717171717 0.0589678239883649
22.2222222222222 0.0562623423868823
22.7272727272727 0.0534335331936687
23.2323232323232 0.0505295175853709
23.7373737373737 0.047592877183394
24.2424242424242 0.0446605805012572
24.7474747474747 0.0417640938101393
25.2525252525253 0.0389296305959111
25.7575757575758 0.0361784994556541
26.2626262626263 0.0335275163324667
26.7676767676768 0.0309894529733437
27.2727272727273 0.0285734991201572
27.7777777777778 0.0262857210275771
28.2828282828283 0.0241295033513034
28.7878787878788 0.022105965236523
29.2929292929293 0.0202143445757572
29.7979797979798 0.01845234694173
30.3030303030303 0.0168164576957933
30.8080808080808 0.0153022172948663
31.3131313131313 0.0139044609404302
31.8181818181818 0.0126175244998089
32.3232323232323 0.0114354191454142
32.8282828282828 0.0103519774577349
33.3333333333333 0.00936097387114379
33.8383838383838 0.00845622234930496
34.3434343434343 0.00763165409331854
34.8484848484849 0.00688137793865916
35.3535353535354 0.00619972590870877
35.8585858585859 0.00558128618068339
36.3636363636364 0.00502092549730741
36.8686868686869 0.00451380283458852
37.3737373737374 0.00405537591959695
37.8787878787879 0.00364140198712576
38.3838383838384 0.00326793397362186
38.8888888888889 0.00293131317259218
39.3939393939394 0.00262815921854744
39.8989898989899 0.00235535812643798
40.4040404040404 0.00211004898992272
40.9090909090909 0.00188960983379207
41.4141414141414 0.00169164302231535
41.9191919191919 0.00151396054495166
42.4242424242424 0.00135456943245482
42.9292929292929 0.00121165749862767
43.4343434343434 0.00108357955459487
43.9393939393939 0.00096884420229457
44.4444444444444 0.000866101280851248
44.949494949495 0.000774130012596597
45.4545454545455 0.000691827873858699
45.959595959596 0.000618200198448275
46.4646464646465 0.000552350508331803
46.969696969697 0.000493471555680199
47.4747474747475 0.000440837052784438
47.979797979798 0.000393794060775234
48.4848484848485 0.000351756004277654
48.989898989899 0.000314196276737588
49.4949494949495 0.00028064239989074
50 0.000250670700467709
};
\addlegendentry{$\mu = 1$, $\sigma=0.3$}
\addplot [very thick, cornflowerblue86180233]
table {%
0 0
0.505050505050505 1.12973482567729e-34
1.01010101010101 1.64585650075935e-23
1.51515151515152 4.69694757421512e-18
2.02020202020202 1.15181880522659e-14
2.52525252525253 2.60324376565289e-12
3.03030303030303 1.44749558123052e-10
3.53535353535354 3.2429281947042e-09
4.04040404040404 3.87215835227825e-08
4.54545454545455 2.92772072039164e-07
5.05050505050505 1.56934417878013e-06
5.55555555555556 6.44471000111058e-06
6.06060606060606 2.14286853372838e-05
6.56565656565657 6.00808154718401e-05
7.07070707070707 0.000146458928566586
7.57575757575758 0.000317807939243284
8.08080808080808 0.000625314934846556
8.58585858585859 0.00113213850142858
9.09090909090909 0.00190861030189384
9.5959595959596 0.00302523392841141
10.1010101010101 0.00454462770513614
10.6060606060606 0.00651374965541447
11.1111111111111 0.00895760946022005
11.6161616161616 0.0118753093000668
12.1212121212121 0.0152387925092694
12.6262626262626 0.0189942334963078
13.1313131313131 0.0230656544103681
13.6363636363636 0.0273601401404505
14.1414141414141 0.0317739435718337
14.6464646464646 0.0361988039638207
15.1515151515152 0.0405279082649442
15.6565656565657 0.0446610726313765
16.1616161616162 0.048508879201401
16.6666666666667 0.0519956493681754
17.1717171717172 0.055061256029149
17.6767676767677 0.0576618676368974
18.1818181818182 0.0597697759744347
18.6868686868687 0.0613724907107481
19.1919191919192 0.0624712921893418
19.6969696969697 0.0630794254411988
20.2020202020202 0.0632200987332096
20.7070707070707 0.0629244239454038
21.2121212121212 0.0622294076032303
21.7171717171717 0.0611760733320378
22.2222222222222 0.0598077707632032
22.7272727272727 0.0581687036256479
23.2323232323232 0.0563026914041509
23.7373737373737 0.0542521645878096
24.2424242424242 0.0520573829171344
24.7474747474747 0.0497558587350315
25.2525252525253 0.0473819630364223
25.7575757575758 0.0449666895544102
26.2626262626263 0.0425375517033479
26.7676767676768 0.0401185879584284
27.2727272727273 0.0377304528907199
27.7777777777778 0.0353905732690101
28.2828282828283 0.0331133511262848
28.7878787878788 0.0309103982717613
29.2929292929293 0.0287907892653647
29.7979797979798 0.0267613222615425
30.3030303030303 0.0248267793106942
30.8080808080808 0.0229901796449125
31.3131313131313 0.0212530211570915
31.8181818181818 0.0196155067110502
32.3232323232323 0.0180767531079567
32.8282828282828 0.0166349815005176
33.3333333333333 0.0152876888143576
33.8383838383838 0.0140318003305042
34.3434343434343 0.0128638040286428
34.8484848484849 0.0117798676113929
35.3535353535354 0.0107759393470904
35.8585858585859 0.00984783400202287
36.3636363636364 0.00899130520002915
36.8686868686869 0.00820210556272424
37.3737373737374 0.00747603595998242
37.8787878787879 0.00680898514825375
38.3838383838384 0.00619696100244609
38.8888888888889 0.00563611446246251
39.3939393939394 0.00512275722357271
39.8989898989899 0.00465337410491465
40.4040404040404 0.00422463093582546
40.9090909090909 0.00383337870778671
41.4141414141414 0.00347665465223425
41.9191919191919 0.00315168082245868
42.4242424242424 0.00285586068199482
42.9292929292929 0.00258677413260771
43.4343434343434 0.00234217135230455
43.9393939393939 0.00211996575761967
44.4444444444444 0.0019182263544752
44.949494949495 0.00173516969786189
45.4545454545455 0.00156915164200068
45.959595959596 0.00141865902909208
46.4646464646465 0.00128230143578002
46.969696969697 0.0011588030715976
47.4747474747475 0.00104699490248499
47.979797979798 0.000945807054557922
48.4848484848485 0.000854261538270645
48.989898989899 0.000771465320598829
49.4949494949495 0.000696603762538634
50 0.000628934430780635
};
\addlegendentry{$\mu = 1.1$, $\sigma=0.3$}
\addplot [semithick, gray, dashed]
table {%
20 -0.00508741986493034
20 0.106835817163537
};
\addlegendentry{true energy}
\end{axis}

\end{tikzpicture}


==> figures/generic_illustration.tex <==
\tikzsetnextfilename{ultrasurface_illustration}%
\begin{tikzpicture}

% Declare a Gaussian function that takes three arguments: (x, mu, sigma)
\pgfmathdeclarefunction{gauss}{3}{%
    \pgfmathparse{1/(#3*sqrt(2*pi))*exp(-((#1-#2)^2)/(2*#3^2))}%
}

% The model function we plot. Expects (x) as the first input and the (alpha) parameter
% that changes the shape as second input. The alpha parameter changes both mean and
% sigma in some linear way.
\pgfmathdeclarefunction{model}{2}{%
  \pgfmathparse{gauss(#1, -0.5 + 0.4 * #2, 0.7 + 0.2 * #2)}%
}

\begin{axis}[
    width=0.6\linewidth,
    ymin=0, ymax=5, zmin=0,
    ytick={1, 2.5, 4},
    yticklabels={-1, 0, 1},
    ylabel=$\Delta \alpha$,
    ztick distance=0.1,
    zlabel=density,
    xlabel=$\Delta \vb{x}$,
    view={50}{30},
    legend columns=2,
    legend cell align={left},
    legend style={/tikz/every even column/.append style={column sep=0.5cm}},
]


    \draw[very thin] (1.3, 0, 0) -- (1.3, 5, 0);


    % We need to draw things "from back to front" to get the correct z-order, that is
    % why we have to draw the systematic sets in the back first, then the nominal set,
    % then the systematic sets in the front. Otherwise, we could have just done this
    % in one single for-loop.

    \pgfplotsinvokeforeach{4, 3.25}{
        \addplot3 [
            tab_orange,
            fill=tab_orange,
            fill opacity=0.5,
            domain=-3.2:3.2,
            samples=100,
            samples y=1,
            forget plot
        ] (x, #1, {model(x, #1)}) \closedcycle;
        \draw[very thin] (1.3, #1, 0) -- (1.3, #1, {model(1.3, #1)});
    }

    \addplot3 [
        area legend,
        tab_blue,
        fill=tab_blue,
        fill opacity=0.5,
        domain=-3.2:3.2,
        samples=100,
        samples y=1
    ] (x, 2.5, {model(x, 2.5)}) \closedcycle;
    \draw[very thin] (1.3, 2.5, 0) -- (1.3, 2.5, {model(1.3, 2.5)});
    \addlegendentry{nominal set}

    \pgfplotsinvokeforeach{1.75,1}{
        \addplot3 [
            tab_orange,
            fill=tab_orange,
            fill opacity=0.5,
            domain=-3.2:3.2,
            samples=100,
            samples y=1,
            forget plot
        ] (x, #1, {model(x, #1)}) \closedcycle;
        \draw[very thin] (1.3, #1, 0) -- (1.3, #1, {model(1.3, #1)});
    }
    \addlegendimage{area legend, tab_orange, fill=tab_orange, fill opacity=0.5}
    \addlegendentry{systematic sets}

    \addplot3 [
        domain=0.7:4.3,
        samples y=1,
        postaction={decorate},
        decoration={markings,
            mark=at position -1 with {\arrowreversed{stealth}},
            mark=at position 1 with {\arrow{stealth}}}
    ] (1.3, x, {model(1.3, x)});
    \addplot3 [only marks, mark size=1, samples y=1, samples at={1, 1.75, 2.5, 3.25, 4}] (1.3, x, {model(1.3, x)});

\end{axis}
\end{tikzpicture}


==> figures/systematic_sets_scale.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{purple}{RGB}{128,0,128}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend columns=2,
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
log basis x={10},
minor xtick={0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9,2,3,4,5,6,7,8,9,20,30,40,50,60,70,80,90,200,300,400,500,600,700,800,900,2000,3000,4000,5000,6000,7000,8000,9000,20000,30000,40000,50000,60000,70000,80000,90000},
minor ytick={},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={reco energy (GeV)},
xmin=8.91250938133745, xmax=112.201845430196,
xmode=log,
xtick style={color=black},
xtick={0.1,1,10,100,1000,10000},
xticklabels={
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\)
},
y grid style={darkgray176},
ylabel={count},
ymin=-14.0675828919181, ymax=400,
ytick style={color=black},
ytick={-50,0,50,100,150,200,250,300,350,400},
xmajorgrids,
xminorgrids,
ymajorgrids
]
\path [draw=purple, fill=purple, opacity=0.5]
(axis cs:10,0)
--(axis cs:10,0)
--(axis cs:10,199.17573908217)
--(axis cs:11.0069417125221,199.17573908217)
--(axis cs:11.0069417125221,217.060919954163)
--(axis cs:12.1152765862859,217.060919954163)
--(axis cs:12.1152765862859,219.022880385629)
--(axis cs:13.3352143216332,219.022880385629)
--(axis cs:13.3352143216332,237.703640088629)
--(axis cs:14.6779926762207,237.703640088629)
--(axis cs:14.6779926762207,220.853900121617)
--(axis cs:16.1559809843987,220.853900121617)
--(axis cs:16.1559809843987,212.520702501444)
--(axis cs:17.7827941003892,212.520702501444)
--(axis cs:17.7827941003892,164.3680513676)
--(axis cs:19.5734178148766,164.3680513676)
--(axis cs:19.5734178148766,128.786048311751)
--(axis cs:21.5443469003188,128.786048311751)
--(axis cs:21.5443469003188,103.608766339569)
--(axis cs:23.7137370566166,103.608766339569)
--(axis cs:23.7137370566166,84.5564931531903)
--(axis cs:26.1015721568254,84.5564931531903)
--(axis cs:26.1015721568254,73.4503131783922)
--(axis cs:28.7298483335366,73.4503131783922)
--(axis cs:28.7298483335366,78.4063939405827)
--(axis cs:31.6227766016838,78.4063939405827)
--(axis cs:31.6227766016838,89.3358727012299)
--(axis cs:34.8070058842841,89.3358727012299)
--(axis cs:34.8070058842841,104.754924513072)
--(axis cs:38.3118684955729,104.754924513072)
--(axis cs:38.3118684955729,121.747337778149)
--(axis cs:42.1696503428582,121.747337778149)
--(axis cs:42.1696503428582,140.835112078627)
--(axis cs:46.4158883361278,140.835112078627)
--(axis cs:46.4158883361278,159.716740300486)
--(axis cs:51.0896977450693,159.716740300486)
--(axis cs:51.0896977450693,170.536385655782)
--(axis cs:56.2341325190349,170.536385655782)
--(axis cs:56.2341325190349,178.088152518533)
--(axis cs:61.896581889126,178.088152518533)
--(axis cs:61.896581889126,175.948899947935)
--(axis cs:68.1292069057961,175.948899947935)
--(axis cs:68.1292069057961,176.257480164579)
--(axis cs:74.9894209332456,176.257480164579)
--(axis cs:74.9894209332456,172.198382439552)
--(axis cs:82.5404185268018,172.198382439552)
--(axis cs:82.5404185268018,164.387807848293)
--(axis cs:90.8517575651687,164.387807848293)
--(axis cs:90.8517575651687,151.333511216929)
--(axis cs:100,151.333511216929)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:100,156.563327090441)
--(axis cs:90.8517575651687,156.563327090441)
--(axis cs:90.8517575651687,169.909124899431)
--(axis cs:82.5404185268018,169.909124899431)
--(axis cs:82.5404185268018,177.910481807121)
--(axis cs:74.9894209332456,177.910481807121)
--(axis cs:74.9894209332456,182.076206796403)
--(axis cs:68.1292069057961,182.076206796403)
--(axis cs:68.1292069057961,181.77813609929)
--(axis cs:61.896581889126,181.77813609929)
--(axis cs:61.896581889126,183.933720136582)
--(axis cs:56.2341325190349,183.933720136582)
--(axis cs:56.2341325190349,176.192546789048)
--(axis cs:51.0896977450693,176.192546789048)
--(axis cs:51.0896977450693,165.130869616176)
--(axis cs:46.4158883361278,165.130869616176)
--(axis cs:46.4158883361278,145.838501605238)
--(axis cs:42.1696503428582,145.838501605238)
--(axis cs:42.1696503428582,126.375034053827)
--(axis cs:38.3118684955729,126.375034053827)
--(axis cs:38.3118684955729,109.143311463492)
--(axis cs:34.8070058842841,109.143311463492)
--(axis cs:34.8070058842841,93.5067527913941)
--(axis cs:31.6227766016838,93.5067527913941)
--(axis cs:31.6227766016838,83.2395803660736)
--(axis cs:28.7298483335366,83.2395803660736)
--(axis cs:28.7298483335366,78.9672665815028)
--(axis cs:26.1015721568254,78.9672665815028)
--(axis cs:26.1015721568254,91.309398117168)
--(axis cs:23.7137370566166,91.309398117168)
--(axis cs:23.7137370566166,112.204718756796)
--(axis cs:21.5443469003188,112.204718756796)
--(axis cs:21.5443469003188,139.356831266552)
--(axis cs:19.5734178148766,139.356831266552)
--(axis cs:19.5734178148766,177.166125923706)
--(axis cs:17.7827941003892,177.166125923706)
--(axis cs:17.7827941003892,227.75654866092)
--(axis cs:16.1559809843987,227.75654866092)
--(axis cs:16.1559809843987,236.807499328961)
--(axis cs:14.6779926762207,236.807499328961)
--(axis cs:14.6779926762207,254.790130533605)
--(axis cs:13.3352143216332,254.790130533605)
--(axis cs:13.3352143216332,235.704925170226)
--(axis cs:12.1152765862859,235.704925170226)
--(axis cs:12.1152765862859,234.143283391227)
--(axis cs:11.0069417125221,234.143283391227)
--(axis cs:11.0069417125221,215.729016931284)
--(axis cs:10,215.729016931284)
--(axis cs:10,0)
--cycle;

\path [draw=steelblue31119180, fill=steelblue31119180, opacity=0.5]
(axis cs:10,0)
--(axis cs:10,0)
--(axis cs:10,175.032504863304)
--(axis cs:11.0069417125221,175.032504863304)
--(axis cs:11.0069417125221,209.231487089794)
--(axis cs:12.1152765862859,209.231487089794)
--(axis cs:12.1152765862859,229.08905830595)
--(axis cs:13.3352143216332,229.08905830595)
--(axis cs:13.3352143216332,262.924308635991)
--(axis cs:14.6779926762207,262.924308635991)
--(axis cs:14.6779926762207,254.966088534631)
--(axis cs:16.1559809843987,254.966088534631)
--(axis cs:16.1559809843987,241.020952511286)
--(axis cs:17.7827941003892,241.020952511286)
--(axis cs:17.7827941003892,223.452254151595)
--(axis cs:19.5734178148766,223.452254151595)
--(axis cs:19.5734178148766,175.739751152218)
--(axis cs:21.5443469003188,175.739751152218)
--(axis cs:21.5443469003188,160.062101905427)
--(axis cs:23.7137370566166,160.062101905427)
--(axis cs:23.7137370566166,122.847215969769)
--(axis cs:26.1015721568254,122.847215969769)
--(axis cs:26.1015721568254,91.9509993298936)
--(axis cs:28.7298483335366,91.9509993298936)
--(axis cs:28.7298483335366,88.0227423317457)
--(axis cs:31.6227766016838,88.0227423317457)
--(axis cs:31.6227766016838,82.2032363642507)
--(axis cs:34.8070058842841,82.2032363642507)
--(axis cs:34.8070058842841,95.4794792668321)
--(axis cs:38.3118684955729,95.4794792668321)
--(axis cs:38.3118684955729,112.444058805512)
--(axis cs:42.1696503428582,112.444058805512)
--(axis cs:42.1696503428582,133.160703810082)
--(axis cs:46.4158883361278,133.160703810082)
--(axis cs:46.4158883361278,153.318118823523)
--(axis cs:51.0896977450693,153.318118823523)
--(axis cs:51.0896977450693,170.329785828714)
--(axis cs:56.2341325190349,170.329785828714)
--(axis cs:56.2341325190349,190.183078221295)
--(axis cs:61.896581889126,190.183078221295)
--(axis cs:61.896581889126,199.817479523768)
--(axis cs:68.1292069057961,199.817479523768)
--(axis cs:68.1292069057961,199.905664514136)
--(axis cs:74.9894209332456,199.905664514136)
--(axis cs:74.9894209332456,199.274827161241)
--(axis cs:82.5404185268018,199.274827161241)
--(axis cs:82.5404185268018,194.76778222157)
--(axis cs:90.8517575651687,194.76778222157)
--(axis cs:90.8517575651687,177.615592373844)
--(axis cs:100,177.615592373844)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:100,183.363901508771)
--(axis cs:90.8517575651687,183.363901508771)
--(axis cs:90.8517575651687,200.848060269091)
--(axis cs:82.5404185268018,200.848060269091)
--(axis cs:82.5404185268018,205.458762916537)
--(axis cs:74.9894209332456,205.458762916537)
--(axis cs:74.9894209332456,206.111760947082)
--(axis cs:68.1292069057961,206.111760947082)
--(axis cs:68.1292069057961,206.011608906412)
--(axis cs:61.896581889126,206.011608906412)
--(axis cs:61.896581889126,196.17943837242)
--(axis cs:56.2341325190349,196.17943837242)
--(axis cs:56.2341325190349,175.917442713231)
--(axis cs:51.0896977450693,175.917442713231)
--(axis cs:51.0896977450693,158.513945326335)
--(axis cs:46.4158883361278,158.513945326335)
--(axis cs:46.4158883361278,137.989832369342)
--(axis cs:42.1696503428582,137.989832369342)
--(axis cs:42.1696503428582,116.903937799258)
--(axis cs:38.3118684955729,116.903937799258)
--(axis cs:38.3118684955729,99.7711477147843)
--(axis cs:34.8070058842841,99.7711477147843)
--(axis cs:34.8070058842841,86.5010519154776)
--(axis cs:31.6227766016838,86.5010519154776)
--(axis cs:31.6227766016838,94.0962974019643)
--(axis cs:28.7298483335366,94.0962974019643)
--(axis cs:28.7298483335366,99.4440867641387)
--(axis cs:26.1015721568254,99.4440867641387)
--(axis cs:26.1015721568254,132.250807586688)
--(axis cs:23.7137370566166,132.250807586688)
--(axis cs:23.7137370566166,171.795586652408)
--(axis cs:21.5443469003188,171.795586652408)
--(axis cs:21.5443469003188,189.032759272255)
--(axis cs:19.5734178148766,189.032759272255)
--(axis cs:19.5734178148766,238.875577320799)
--(axis cs:17.7827941003892,238.875577320799)
--(axis cs:17.7827941003892,257.468046139608)
--(axis cs:16.1559809843987,257.468046139608)
--(axis cs:16.1559809843987,272.459370792436)
--(axis cs:14.6779926762207,272.459370792436)
--(axis cs:14.6779926762207,281.351657838362)
--(axis cs:13.3352143216332,281.351657838362)
--(axis cs:13.3352143216332,246.594642070832)
--(axis cs:12.1152765862859,246.594642070832)
--(axis cs:12.1152765862859,226.365491210868)
--(axis cs:11.0069417125221,226.365491210868)
--(axis cs:11.0069417125221,191.006361333216)
--(axis cs:10,191.006361333216)
--(axis cs:10,0)
--cycle;

\path [draw=darkorange25512714, fill=darkorange25512714, opacity=0.5]
(axis cs:10,0)
--(axis cs:10,0)
--(axis cs:10,205.761361871886)
--(axis cs:11.0069417125221,205.761361871886)
--(axis cs:11.0069417125221,203.65312743136)
--(axis cs:12.1152765862859,203.65312743136)
--(axis cs:12.1152765862859,197.352212331513)
--(axis cs:13.3352143216332,197.352212331513)
--(axis cs:13.3352143216332,189.362119254433)
--(axis cs:14.6779926762207,189.362119254433)
--(axis cs:14.6779926762207,175.5256025956)
--(axis cs:16.1559809843987,175.5256025956)
--(axis cs:16.1559809843987,145.915572423188)
--(axis cs:17.7827941003892,145.915572423188)
--(axis cs:17.7827941003892,112.059151572744)
--(axis cs:19.5734178148766,112.059151572744)
--(axis cs:19.5734178148766,93.6122327693099)
--(axis cs:21.5443469003188,93.6122327693099)
--(axis cs:21.5443469003188,80.4592482315404)
--(axis cs:23.7137370566166,80.4592482315404)
--(axis cs:23.7137370566166,67.7756473041824)
--(axis cs:26.1015721568254,67.7756473041824)
--(axis cs:26.1015721568254,72.4615186251053)
--(axis cs:28.7298483335366,72.4615186251053)
--(axis cs:28.7298483335366,80.4801892004395)
--(axis cs:31.6227766016838,80.4801892004395)
--(axis cs:31.6227766016838,93.9453023610925)
--(axis cs:34.8070058842841,93.9453023610925)
--(axis cs:34.8070058842841,114.102305549798)
--(axis cs:38.3118684955729,114.102305549798)
--(axis cs:38.3118684955729,129.985631746474)
--(axis cs:42.1696503428582,129.985631746474)
--(axis cs:42.1696503428582,144.34156826583)
--(axis cs:46.4158883361278,144.34156826583)
--(axis cs:46.4158883361278,153.21369800081)
--(axis cs:51.0896977450693,153.21369800081)
--(axis cs:51.0896977450693,161.29875323007)
--(axis cs:56.2341325190349,161.29875323007)
--(axis cs:56.2341325190349,168.672133364476)
--(axis cs:61.896581889126,168.672133364476)
--(axis cs:61.896581889126,161.765885987995)
--(axis cs:68.1292069057961,161.765885987995)
--(axis cs:68.1292069057961,155.128449593658)
--(axis cs:74.9894209332456,155.128449593658)
--(axis cs:74.9894209332456,145.707860733053)
--(axis cs:82.5404185268018,145.707860733053)
--(axis cs:82.5404185268018,133.650518740095)
--(axis cs:90.8517575651687,133.650518740095)
--(axis cs:90.8517575651687,122.130186967586)
--(axis cs:100,122.130186967586)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:100,126.728203439491)
--(axis cs:90.8517575651687,126.728203439491)
--(axis cs:90.8517575651687,138.564824044685)
--(axis cs:82.5404185268018,138.564824044685)
--(axis cs:82.5404185268018,150.91339491808)
--(axis cs:74.9894209332456,150.91339491808)
--(axis cs:74.9894209332456,160.555544379444)
--(axis cs:68.1292069057961,160.555544379444)
--(axis cs:68.1292069057961,167.349911968588)
--(axis cs:61.896581889126,167.349911968588)
--(axis cs:61.896581889126,174.386032000935)
--(axis cs:56.2341325190349,174.386032000935)
--(axis cs:56.2341325190349,166.863239919776)
--(axis cs:51.0896977450693,166.863239919776)
--(axis cs:51.0896977450693,158.601238341765)
--(axis cs:46.4158883361278,158.601238341765)
--(axis cs:46.4158883361278,149.520271873034)
--(axis cs:42.1696503428582,149.520271873034)
--(axis cs:42.1696503428582,134.850661780842)
--(axis cs:38.3118684955729,134.850661780842)
--(axis cs:38.3118684955729,118.58764801433)
--(axis cs:34.8070058842841,118.58764801433)
--(axis cs:34.8070058842841,97.9803523539387)
--(axis cs:31.6227766016838,97.9803523539387)
--(axis cs:31.6227766016838,84.5604656770365)
--(axis cs:28.7298483335366,84.5604656770365)
--(axis cs:28.7298483335366,77.0220824292516)
--(axis cs:26.1015721568254,77.0220824292516)
--(axis cs:26.1015721568254,72.6869765603297)
--(axis cs:23.7137370566166,72.6869765603297)
--(axis cs:23.7137370566166,87.2198628029088)
--(axis cs:21.5443469003188,87.2198628029088)
--(axis cs:21.5443469003188,101.900734942572)
--(axis cs:19.5734178148766,101.900734942572)
--(axis cs:19.5734178148766,121.676834800016)
--(axis cs:17.7827941003892,121.676834800016)
--(axis cs:17.7827941003892,157.70142880867)
--(axis cs:16.1559809843987,157.70142880867)
--(axis cs:16.1559809843987,189.303242993783)
--(axis cs:14.6779926762207,189.303242993783)
--(axis cs:14.6779926762207,204.118899869635)
--(axis cs:13.3352143216332,204.118899869635)
--(axis cs:13.3352143216332,212.711547177021)
--(axis cs:12.1152765862859,212.711547177021)
--(axis cs:12.1152765862859,219.679297368581)
--(axis cs:11.0069417125221,219.679297368581)
--(axis cs:11.0069417125221,222.418416304474)
--(axis cs:10,222.418416304474)
--(axis cs:10,0)
--cycle;

\addplot [very thick, purple]
table {%
10 0
10 207.452378006727
11.0069417125221 207.452378006727
11.0069417125221 225.602101672695
12.1152765862859 225.602101672695
12.1152765862859 227.363902777927
13.3352143216332 227.363902777927
13.3352143216332 246.246885311117
14.6779926762207 246.246885311117
14.6779926762207 228.830699725289
16.1559809843987 228.830699725289
16.1559809843987 220.138625581182
17.7827941003892 220.138625581182
17.7827941003892 170.767088645653
19.5734178148766 170.767088645653
19.5734178148766 134.071439789152
21.5443469003188 134.071439789152
21.5443469003188 107.906742548182
23.7137370566166 107.906742548182
23.7137370566166 87.9329456351792
26.1015721568254 87.9329456351792
26.1015721568254 76.2087898799475
28.7298483335366 76.2087898799475
28.7298483335366 80.8229871533282
31.6227766016838 80.8229871533282
31.6227766016838 91.421312746312
34.8070058842841 91.421312746312
34.8070058842841 106.949117988282
38.3118684955729 106.949117988282
38.3118684955729 124.061185915988
42.1696503428582 124.061185915988
42.1696503428582 143.336806841933
46.4158883361278 143.336806841933
46.4158883361278 162.423804958331
51.0896977450693 162.423804958331
51.0896977450693 173.364466222415
56.2341325190349 173.364466222415
56.2341325190349 181.010936327557
61.896581889126 181.010936327557
61.896581889126 178.863518023613
68.1292069057961 178.863518023613
68.1292069057961 179.166843480491
74.9894209332456 179.166843480491
74.9894209332456 175.054432123336
82.5404185268018 175.054432123336
82.5404185268018 167.148466373862
90.8517575651687 167.148466373862
90.8517575651687 153.948419153685
100 153.948419153685
100 0
};
\addlegendentry{nominal}
\addplot [very thick, steelblue31119180]
table {%
10 0
10 183.01943309826
11.0069417125221 183.01943309826
11.0069417125221 217.798489150331
12.1152765862859 217.798489150331
12.1152765862859 237.841850188391
13.3352143216332 237.841850188391
13.3352143216332 272.137983237177
14.6779926762207 272.137983237177
14.6779926762207 263.712729663533
16.1559809843987 263.712729663533
16.1559809843987 249.244499325447
17.7827941003892 249.244499325447
17.7827941003892 231.163915736197
19.5734178148766 231.163915736197
19.5734178148766 182.386255212236
21.5443469003188 182.386255212236
21.5443469003188 165.928844278917
23.7137370566166 165.928844278917
23.7137370566166 127.549011778229
26.1015721568254 127.549011778229
26.1015721568254 95.6975430470162
28.7298483335366 95.6975430470162
28.7298483335366 91.059519866855
31.6227766016838 91.059519866855
31.6227766016838 84.3521441398641
34.8070058842841 84.3521441398641
34.8070058842841 97.6253134908082
38.3118684955729 97.6253134908082
38.3118684955729 114.673998302385
42.1696503428582 114.673998302385
42.1696503428582 135.575268089712
46.4158883361278 135.575268089712
46.4158883361278 155.916032074929
51.0896977450693 155.916032074929
51.0896977450693 173.123614270973
56.2341325190349 173.123614270973
56.2341325190349 193.181258296858
61.896581889126 193.181258296858
61.896581889126 202.91454421509
68.1292069057961 202.91454421509
68.1292069057961 203.008712730609
74.9894209332456 203.008712730609
74.9894209332456 202.366795038889
82.5404185268018 202.366795038889
82.5404185268018 197.80792124533
90.8517575651687 197.80792124533
90.8517575651687 180.489746941308
100 180.489746941308
100 0
};
\addlegendentry{$\mu = 1.1$, $\sigma=0.3$}
\addplot [very thick, darkorange25512714]
table {%
10 0
10 214.08988908818
11.0069417125221 214.08988908818
11.0069417125221 211.666212399971
12.1152765862859 211.666212399971
12.1152765862859 205.031879754267
13.3352143216332 205.031879754267
13.3352143216332 196.740509562034
14.6779926762207 196.740509562034
14.6779926762207 182.414422794692
16.1559809843987 182.414422794692
16.1559809843987 151.808500615929
17.7827941003892 151.808500615929
17.7827941003892 116.86799318638
19.5734178148766 116.86799318638
19.5734178148766 97.7564838559411
21.5443469003188 97.7564838559411
21.5443469003188 83.8395555172246
23.7137370566166 83.8395555172246
23.7137370566166 70.231311932256
26.1015721568254 70.231311932256
26.1015721568254 74.7418005271784
28.7298483335366 74.7418005271784
28.7298483335366 82.520327438738
31.6227766016838 82.520327438738
31.6227766016838 95.9628273575156
34.8070058842841 95.9628273575156
34.8070058842841 116.344976782064
38.3118684955729 116.344976782064
38.3118684955729 132.418146763658
42.1696503428582 132.418146763658
42.1696503428582 146.930920069432
46.4158883361278 146.930920069432
46.4158883361278 155.907468171287
51.0896977450693 155.907468171287
51.0896977450693 164.080996574923
56.2341325190349 164.080996574923
56.2341325190349 171.529082682706
61.896581889126 171.529082682706
61.896581889126 164.557898978292
68.1292069057961 164.557898978292
68.1292069057961 157.841996986551
74.9894209332456 157.841996986551
74.9894209332456 148.310627825567
82.5404185268018 148.310627825567
82.5404185268018 136.10767139239
90.8517575651687 136.10767139239
90.8517575651687 124.429195203538
100 124.429195203538
100 0
};
\addlegendentry{$\mu = 0.9$, $\sigma=0.3$}
\end{axis}

\end{tikzpicture}


